The Task Shield: Enforcing Task Alignment to Defend Against Indirect Prompt Injection in LLM Agents

Large Language Model (LLM) agents are increasingly being deployed as conversational assistants capable of performing complex real-world tasks through tool integration. This enhanced ability to interact with external systems and process various data sources, while powerful, introduces significant security vulnerabilities. In particular, indirect prompt injection attacks pose a critical threat, where malicious instructions embedded within external data sources can manipulate agents to deviate from user intentions. While existing defenses based on rule constraints, source spotlighting, and authentication protocols show promise, they struggle to maintain robust security while preserving task functionality. We propose a novel and orthogonal perspective that reframes agent security from preventing harmful actions to ensuring task alignment, requiring every agent action to serve user objectives. Based on this insight, we develop Task Shield, a test-time defense mechanism that systematically verifies whether each instruction and tool call contributes to user-specified goals. Through experiments on the AgentDojo benchmark, we demonstrate that Task Shield reduces attack success rates (2.07\%) while maintaining high task utility (69.79\%) on GPT-4o.

==> UserGoalShield/Tables/4o_full_results.tex <==
\begin{table*}[htbp]
    \centering
    \small 
    \setlength{\tabcolsep}{2pt} 
    \renewcommand{\arraystretch}{1.3} 
    \begin{tabular}{lccc|ccc|ccc|ccc|ccc}
        \toprule
        \textbf{Suite} & \multicolumn{3}{c|}{\textbf{Travel}} & \multicolumn{3}{c|}{\textbf{Workspace}} & \multicolumn{3}{c|}{\textbf{Banking}} & \multicolumn{3}{c|}{\textbf{Slack}} & \multicolumn{3}{c}{\textbf{Overall}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
        \textbf{Defense} & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ \\
        \midrule
    No Defense & 65.00 & 64.29 & 11.43 & \underline{62.50} & 24.17 & 40.42 & 75.00 & 69.44 & 62.50 & \textbf{80.95} & \underline{63.81} & 92.38 & 69.07 & 50.08 & 47.69 \\
Tool Filter & \textbf{90.00} & 70.00 & 5.71 & 55.00 & 51.67 & \underline{4.17} & \underline{81.25} & 56.94 & 11.11 & \textbf{80.95} & 47.62 & \underline{8.57} & 72.16 & 56.28 & \underline{6.84} \\
Repeat Prompt & \textbf{90.00} & \underline{72.14} & 7.14 & \textbf{80.00} & \underline{60.42} & 14.58 & \textbf{93.75} & \underline{77.08} & 46.53 & \textbf{80.95} & 62.86 & 60.00 & \textbf{84.54} & \underline{67.25} & 27.82 \\
Delimiting & 75.00 & \underline{72.14} & 3.57 & \underline{62.50} & 30.42 & 35.00 & \underline{81.25} & \underline{77.08} & 61.81 & \textbf{80.95} & 61.90 & 80.00 & 72.16 & 55.64 & 41.65 \\
PI Detector & 30.00 & 16.43 & \textbf{0.00} & 52.50 & 15.83 & 15.00 & 43.75 & 31.25 & \textbf{0.69} & \underline{28.57} & 25.71 & 12.38 & 41.24 & 21.14 & 7.95 \\
Task Shield & \underline{80.00} & \textbf{72.86} & \underline{1.43} & \underline{62.50} & \textbf{62.50} & \textbf{0.42} & \underline{81.25} & \textbf{82.64} & \underline{6.25} & \textbf{80.95} & \textbf{64.76} & \textbf{0.95} & \underline{73.20} & \textbf{69.79} & \textbf{2.07} \\

        \bottomrule
    \end{tabular}
    \caption{Defense performance against Important Messages attack for the GPT-4o model. Results are reported across Clean Utility (CU), Utility under Attack (U), and Attack Success Rate (ASR) across task suites. Bold values denote the best-performing results for each metric, while underlined values indicate the second-best performance.}
    \label{tab:performance_comparison_4o}
\end{table*}
    

==> UserGoalShield/Tables/4omini_full_results.tex <==
% \begin{table*}[htbp]
%     \centering
%     \small 
%     \setlength{\tabcolsep}{2pt} 
%     \renewcommand{\arraystretch}{1.3} 
%     \begin{tabular}{lccc|ccc|ccc|ccc|ccc}
%         \toprule
%         \textbf{Suite} & \multicolumn{3}{c|}{\textbf{Travel}} & \multicolumn{3}{c|}{\textbf{Workspace}} & \multicolumn{3}{c|}{\textbf{Banking}} & \multicolumn{3}{c|}{\textbf{Slack}} & \multicolumn{3}{c}{\textbf{Overall}} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
%         \textbf{Defense} & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ \\
%         \midrule
%     No Defense & 55.00 & 47.14 & 13.57 & \underline{82.50} & 59.17 & 17.92 & \textbf{50.00} & 38.19 & 34.03 & \underline{66.67} & 48.57 & 57.14 & \textbf{68.04} & 49.92 & 27.19 \\
% Tool Filter & \underline{60.00} & \textbf{58.57} & \underline{0.71} & 70.00 & \underline{64.58} & \underline{2.50} & \textbf{50.00} & \underline{43.06} & \underline{11.11} & 57.14 & 45.71 & \underline{7.62} & 61.86 & \textbf{55.17} & \underline{4.93} \\
% Repeat Prompt & \textbf{70.00} & \underline{54.29} & \textbf{0.00} & 70.00 & 61.25 & 8.33 & \underline{43.75} & \textbf{43.75} & 17.36 & \textbf{71.43} & 33.33 & 13.33 & \underline{65.98} & 51.03 & 9.38 \\
% Delimiting & \underline{60.00} & 52.14 & 7.14 & 72.50 & \underline{64.58} & 12.92 & \underline{43.75} & 35.42 & 33.33 & \textbf{71.43} & \textbf{56.19} & 48.57 & 64.95 & 53.74 & 22.26 \\
% Task Shield & 55.00 & 49.29 & \underline{0.71} & \textbf{85.00} & \textbf{69.58} & \textbf{1.25} & \underline{43.75} & 37.50 & \textbf{6.25} & \underline{66.67} & \underline{50.48} & \textbf{0.95} & \textbf{68.04} & \underline{54.53} & \textbf{2.23} \\

%         \bottomrule
%     \end{tabular}
%     \caption{Defense performance against Important Messages attack for the GPT-4o-mini model. Results are reported across Clean Utility (CU), Utility under Attack (U), and Attack Success Rate (ASR) across task suites. Bold values denote the best-performing results for each metric, while underlined values indicate the second-best performance.}
%     \label{tab:performance_comparison_4omini}
% \end{table*}

\begin{table*}[htbp]
    \centering
    \small 
    \setlength{\tabcolsep}{2pt} 
    \renewcommand{\arraystretch}{1.3} 
    \begin{tabular}{lccc|ccc|ccc|ccc|ccc}
        \toprule
        \textbf{Suite} & \multicolumn{3}{c|}{\textbf{Travel}} & \multicolumn{3}{c|}{\textbf{Workspace}} & \multicolumn{3}{c|}{\textbf{Banking}} & \multicolumn{3}{c|}{\textbf{Slack}} & \multicolumn{3}{c}{\textbf{Overall}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
        \textbf{Defense} & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ & CU$\uparrow$ & U$\uparrow$ & ASR$\downarrow$ \\
        \midrule
    No Defense & 55.00 & 47.14 & 13.57 & \underline{82.50} & 59.17 & 17.92 & \textbf{50.00} & 38.19 & 34.03 & \underline{66.67} & 48.57 & 57.14 & \textbf{68.04} & 49.92 & 27.19 \\
Tool Filter & \underline{60.00} & \textbf{58.57} & \underline{0.71} & 70.00 & \underline{64.58} & \underline{2.50} & \textbf{50.00} & \underline{43.06} & 11.11 & 57.14 & 45.71 & \underline{7.62} & 61.86 & \textbf{55.17} & \underline{4.93} \\
Repeat Prompt & \textbf{70.00} & \underline{54.29} & \textbf{0.00} & 70.00 & 61.25 & 8.33 & \underline{43.75} & \textbf{43.75} & 17.36 & \textbf{71.43} & 33.33 & 13.33 & \underline{65.98} & 51.03 & 9.38 \\
Delimiting & \underline{60.00} & 52.14 & 7.14 & 72.50 & \underline{64.58} & 12.92 & \underline{43.75} & 35.42 & 33.33 & \textbf{71.43} & \textbf{56.19} & 48.57 & 64.95 & 53.74 & 22.26 \\
PI Detector & 25.00 & 14.29 & \textbf{0.00} & 60.00 & 27.50 & 12.92 & 37.50 & 29.86 & \underline{10.42} & 23.81 & 15.24 & \underline{7.62} & 41.24 & 23.05 & 8.59 \\
Task Shield & 55.00 & 49.29 & \underline{0.71} & \textbf{85.00} & \textbf{69.58} & \textbf{1.25} & \underline{43.75} & 37.50 & \textbf{6.25} & \underline{66.67} & \underline{50.48} & \textbf{0.95} & \textbf{68.04} & \underline{54.53} & \textbf{2.23} \\

        \bottomrule
    \end{tabular}
    \caption{Defense performance against Important Messages attack for the GPT-4o-mini model. Results are reported across Clean Utility (CU), Utility under Attack (U), and Attack Success Rate (ASR) across task suites. Bold values denote the best-performing results for each metric, while underlined values indicate the second-best performance.}
    \label{tab:performance_comparison_4omini}
\end{table*}
    

==> UserGoalShield/app-extended_related_work.tex <==
\subsection{Extended Related Work}

\paragraph{LLM Agent and Tool Using}
\todo{usage}
\paragraph{Prompt Injection}
Direct injection
Indirect injection 

\paragraph{Prompt Injection Defense}
black-box

white-box


\paragraph{Prompt Injection Benchmarks}
InjecAgent~\cite{zhan2024injecagent}

\paragraph{Guard Agent}

Our method is othogonal to the guard agents....
